SN 2022oqm -- a Ca-rich explosion of a compact progenitor embedded in C/O circumstellar material

We present the discovery and analysis of SN\,2022oqm, a Type Ic supernova (SN) detected $<1$\,day after explosion. The SN rises to a blue and short-lived (2\,days) initial peak. Early-time spectral observations of SN\,2022oqm show a hot (40,000\,K) continuum with high-ionization C and O absorption features at velocities of 4000\,km\,s$^{-1}$, while its photospheric radius expands at 20,000\,\kms, indicating a pre-existing distribution of expanding C/O material. After $\sim2.5$\,days, both the spectrum and light curves evolve into those of a typical SN Ic, with line velocities of $\sim10,000$\,km\,s$^{-1}$, in agreement with the photospheric radius evolution. The optical light curves reach a second peak at $t\approx15$\,days. By $t=60$\,days, the spectrum of \oqm\ becomes nearly nebular, displaying strong \ion{Ca}{2} and [\ion{Ca}{2}] emission with no detectable [\ion{O}{1}], marking this event as Ca-rich. The early behavior can be explained by $10^{-3}$\,\msun\ of optically thin circumstellar material (CSM) surrounding either (1) a massive compact progenitor such as a Wolf-Rayet star, (2) a massive stripped progenitor with an extended envelope, or (3) a binary system with a white dwarf. We propose that the early-time light curve is powered by both interaction of the ejecta with the optically thin CSM and shock cooling (in the massive-star scenario). The observations can be explained by CSM that is optically thick to X-ray photons, is optically thick in the lines as seen in the spectra, and is optically thin to visible-light continuum photons that come either from downscattered X-rays or from the shock-heated ejecta. Calculations show that this scenario is self-consistent.

==> bb_fits.tex <==
\begin{deluxetable*}{cccccccc}
\label{tab:bb_fits}

\centering

\tablecaption{Blackbody evolution of SN\,2022oqm}
\tablewidth{28pt} 

\tablehead{\colhead{JD} & \colhead{t [rest-frame days]} & \colhead{$\rm T_{eff}\ [^{\circ} \rm K]$} & \colhead{$\rm R_{BB}\ [10^{14} \rm cm]$ } & \colhead{$\rm L_{BB}\ [10^{42} \rm erg\ \rm s^{-1}]$} & \colhead{$\rm L_{pseudo}\ [10^{42} \rm erg\ \rm s^{-1}]$} & \colhead{$\rm L_{pseudo,extrap}\  [10^{42} \rm erg\ \rm s^{-1}]$} & \colhead{$\chi^{2}/dof$}} 

\tabletypesize{\scriptsize} 
\startdata
2459772.04 & 0.82 & $37000\pm13800$ & $1.44\pm0.41$ & $27.83\pm25.9$ & $3.02\pm3.02$ & $28.28\pm23.51$ & 10.6 \\
2459772.77 & 1.54 & $16900\pm700$ & $2.91\pm0.14$ & $4.93\pm0.37$ & $2.91\pm2.91$ & $4.88\pm0.15$ & 3.94 \\
2459773.18 & 1.94 & $12000\pm200$ & $4.29\pm0.11$ & $2.7\pm0.07$ & $2.19\pm2.19$ & $2.79\pm0.02$ & 1.71 \\
2459774.22 & 2.97 & $9400\pm200$ & $6.43\pm0.2$ & $2.33\pm0.06$ & $2.01\pm2.01$ & $2.44\pm0.01$ & 2.61 \\
2459774.74 & 3.48 & $8900\pm200$ & $7.44\pm0.27$ & $2.43\pm0.07$ & $2.13\pm2.13$ & $2.59\pm0.01$ & 3.57 \\
2459775.27 & 4.0 & $8300\pm200$ & $8.48\pm0.35$ & $2.48\pm0.08$ & $2.17\pm2.17$ & $2.66\pm0.02$ & 6.01 \\
2459776.55 & 5.28 & $7700\pm100$ & $10.28\pm0.41$ & $2.64\pm0.08$ & $2.23\pm2.23$ & $2.8\pm0.02$ & 5.8 \\
2459777.75 & 6.46 & $7500\pm100$ & $11.11\pm0.47$ & $2.74\pm0.08$ & $2.26\pm2.26$ & $2.89\pm0.02$ & 4.88 \\
2459779.17 & 7.87 & $7000\pm100$ & $12.66\pm0.53$ & $2.74\pm0.09$ & $2.15\pm2.15$ & $2.84\pm0.02$ & 5.23 \\
2459779.78 & 8.47 & $6800\pm100$ & $13.59\pm0.67$ & $2.74\pm0.11$ & $2.11\pm2.11$ & $2.84\pm0.03$ & 8.16 \\
2459783.62 & 12.27 & $6300\pm100$ & $15.95\pm0.7$ & $2.87\pm0.09$ & $2.13\pm2.13$ & $2.99\pm0.03$ & 6.11 \\
2459787.15 & 15.75 & $5800\pm100$ & $18.38\pm0.92$ & $2.68\pm0.1$ & $1.84\pm1.84$ & $2.78\pm0.03$ & 5.43 \\
2459790.0 & 18.57 & $5300\pm200$ & $20.35\pm1.51$ & $2.39\pm0.11$ & $1.43\pm1.43$ & $2.49\pm0.05$ & 8.23 \\
2459793.0 & 21.54 & $5200\pm200$ & $20.31\pm1.5$ & $2.07\pm0.09$ & $1.18\pm1.18$ & $2.13\pm0.04$ & 6.47 \\
2459796.0 & 24.51 & $5200\pm200$ & $18.09\pm1.23$ & $1.69\pm0.06$ & $0.94\pm0.94$ & $1.72\pm0.03$ & 4.04 \\
2459799.0 & 27.47 & $4900\pm100$ & $18.5\pm1.22$ & $1.4\pm0.05$ & $0.69\pm0.69$ & $1.45\pm0.03$ & 3.0 \\
2459802.0 & 30.44 & $4700\pm100$ & $18.88\pm1.25$ & $1.19\pm0.04$ & $0.54\pm0.54$ & $1.24\pm0.03$ & 2.83 \\
2459805.0 & 33.41 & $4600\pm100$ & $18.16\pm1.21$ & $1.02\pm0.04$ & $0.45\pm0.45$ & $1.05\pm0.02$ & 2.73 \\
2459807.0 & 35.38 & $4600\pm100$ & $17.01\pm0.98$ & $0.91\pm0.03$ & $0.39\pm0.39$ & $0.93\pm0.02$ & 2.06 \\
2459809.0 & 37.36 & $4600\pm100$ & $16.26\pm1.01$ & $0.83\pm0.03$ & $0.36\pm0.36$ & $0.85\pm0.02$ & 2.32 \\
2459813.0 & 41.32 & $4500\pm100$ & $15.01\pm1.07$ & $0.68\pm0.03$ & $0.28\pm0.28$ & $0.68\pm0.02$ & 2.5 \\
2459817.0 & 45.27 & $4600\pm200$ & $12.74\pm1.13$ & $0.52\pm0.03$ & $0.19\pm0.19$ & $0.53\pm0.02$ & 2.04 \\
2459820.0 & 48.24 & $4600\pm200$ & $11.26\pm1.04$ & $0.41\pm0.02$ & $0.16\pm0.16$ & $0.42\pm0.01$ & 1.99 \\
2459824.0 & 52.19 & $4600\pm200$ & $9.43\pm1.1$ & $0.29\pm0.02$ & $0.09\pm0.09$ & $0.29\pm0.01$ & 2.23 \\
2459837.5 & 65.54 & $1650\pm20$ & $44.4\pm1.3$ & $0.1\pm0.002$ & $0.09\pm0.002$ & $0.17\pm0.01$ & 0.2 \\
\hline
\enddata
\tablenotetext{a}{A 0.1 mag systematic error was assumed when performing the fits.}
\tablenotetext{b}{After $t=40$ days, we consider the blackbody fits and extrapolation to the IR and UV as unreliable, since the spectrum becomes line-dominated. We report the values here for completeness.}
\tablenotetext{c}{The last epoch is fit only to the $JHK$, but integrated using all observed bands, as discussed in the text.}
\end{deluxetable*}




==> phot.tex <==
\begin{deluxetable*}{ccllc}
\label{tab:phot}

\centering

\tablecaption{Log of photometric observations (truncated)}
\tablewidth{24pt} 

\tablehead{\colhead{JD} & \colhead{t [rest-frame days]} & \colhead{Instrument} & \colhead{Filter} & \colhead{AB Magnitude}} 
\tabletypesize{\scriptsize} 
\startdata
2459771.7 & 0.47 & ZTF/P48 & \textit{g} & $17.23 \pm 0.02$ \\
2459771.81 & 1.47 & P60/SEDM & \textit{r} & $17.34 \pm 0.02$ \\
2459771.83 & 1.51 & P60/SEDM & \textit{g} & $17.03 \pm 0.03$ \\
2459771.84 & 1.53 & P60/SEDM & \textit{r} & $17.35 \pm 0.02$ \\
2459771.84 & 2.53 & P60/SEDM & \textit{i} & $17.66 \pm 0.03$ \\
2459772.04 & 3.44 & Swift/UVOT & \textit{W1} & $16.04 \pm 0.04$ \\
2459772.04 & 3.51 & Swift/UVOT & \textit{U} & $16.26 \pm 0.04$ \\
2459772.04 & 3.58 & Swift/UVOT & \textit{B} & $16.47 \pm 0.06$ \\
2459772.04 & 4.47 & Swift/UVOT & \textit{W2} & $15.88 \pm 0.03$ \\
2459772.05 & 5.46 & Swift/UVOT & \textit{V} & $16.85 \pm 0.11$ \\
2459772.05 & 5.5 & Swift/UVOT & \textit{M2} & $15.88 \pm 0.03$ \\
2459772.39 & 5.54 & LT/IO:O & \textit{g} & $16.91 \pm 0.08$ \\
2459772.39 & 8.43 & LT/IO:O & \textit{r} & $17.17 \pm 0.05$ \\
2459772.39 & 8.51 & LT/IO:O & \textit{i} & $17.51 \pm 0.07$ \\
2459772.39 & 10.43 & LT/IO:O & \textit{u} & $16.62 \pm 0.06$ \\
2459772.39 & 11.37 & LT/IO:O & \textit{z} & $17.78 \pm 0.09$ \\

\enddata

\tablenotetext{a}{All measurements are reported in the AB system and are corrected for Galactic line-of-sight reddening.}
\tablenotetext{b}{The full table will be made available electronically on WISeREP upon publication.}
\vspace{-0.15cm}

\end{deluxetable*}

==> powerlaw_fits.tex <==
\begin{deluxetable*}{ccccccccc}
\label{tab:pl_fits}

\centering

\tablecaption{Power law fits for the early blackbody evolution SN\,2022oqm}
\tablewidth{24pt} 



\tablehead{\colhead{$T_{0}\ [^{\circ} \rm K]$}&\colhead{$R_{0}\ [10^{14} \rm cm]$}&\colhead{$\alpha$}&\colhead{$\beta$}&\colhead{$t_{exp}\ [JD]$}&\colhead{$t_{br}$ [rest days]} & \colhead{$\alpha_{2}$}} 
\tabletypesize{\scriptsize} 
\startdata
$22000\pm4000$ & ${ 2.7}^{+ 0.5}_{- 1.4}$  & ${-1.0}^{+ 0.1}_{- 0.2}$  & ${ 0.9}^{+ 0.3}_{-0.1}$ & ${ 2459771.2}^{+ 0.2}_{- 0.2} $ & ${ 2.2}^{+ 0.2}_{- 0.3} $  & $ {-0.3}^{+0.1}_{- 0.1} $\\
\hline
\enddata
\tablenotetext{a}{A 0.1 mag systematic error was assumed when performing the fits.}
\tablenotetext{b}{In our best fit, $\beta_{2}=\beta$. Thus, we do not report $\beta_{2}$ or $t_{br,2}$}


\end{deluxetable*}


==> spectra_log.tex <==

\begin{deluxetable}{lcccc}
\tablecaption{Summary of Spectroscopic Observations of SN 2022oqm \label{tab:spec}}
\tablecolumns{5}
\tabletypesize{\footnotesize}  %\small
\tablehead{
\colhead{Start Date (UTC)} &
\colhead{Phase (d)} &
\colhead{Telescope} &
\colhead{Spectrograph} &
\colhead{Exp (s)}
}
\startdata 
2022-07-11.312 &  0.596 &       P60 &       SEDM &    1800 \\
2022-07-11.418 &  0.701 &  Gemini-N &       GMOS &    3600 \\
2022-07-11.913 &  1.196 &       NOT &     ALFOSC &    1800 \\
2022-07-12.214 &  1.497 &       P60 &       SEDM &    1800 \\
2022-07-12.980 &  2.263 &        LT &      SPRAT &     750 \\
2022-07-13.178 &  2.462 &       P60 &       SEDM &    1800 \\
2022-07-13.915 &  3.199 &       NOT &     ALFOSC &    1800 \\
2022-07-14.220 &  3.503 &       P60 &       SEDM &    1800 \\
2022-07-15.891 &  5.174 &       NOT &     ALFOSC &     600 \\
2022-07-17.177 &  6.460 &       P60 &       SEDM &    1800 \\
2022-07-17.989 &  7.273 &       NOT &     ALFOSC &    1800 \\
2022-07-18.183 &  7.466 &       P60 &       SEDM &    1800 \\
2022-07-20.175 &  9.459 &       P60 &       SEDM &    1800 \\
2022-07-21.234 & 10.518 &     Shane &       Kast &    2160/2100 \\
2022-07-21.271 & 10.555 &  Gemini-N &       GMOS &    1600 \\
2022-07-22.319 & 11.603 &      P200 &       DBSP &     300 \\
2022-07-25.303 & 14.587 &     Shane &       Kast &    1860/1800 \\
2022-07-26.174 & 15.458 &       P60 &       SEDM &    1800 \\
2022-07-27.241 & 16.524 &       P60 &       SEDM &    1800 \\
2022-07-27.933 & 17.217 &       NOT &     ALFOSC &    1200 \\
2022-07-29.195 & 18.479 &     Shane &       Kast &    1860/2100 \\
2022-08-05.187 & 25.470 &     Shane &       Kast &    2460/2400 \\
2022-08-07.164 & 27.448 &       P60 &       SEDM &    1800 \\
2022-08-10.189 & 30.473 &       P60 &       SEDM &    1800 \\
2022-08-14.161 & 34.444 &       P60 &       SEDM &    1800 \\
2022-08-15.878 & 36.162 &       NOT &     ALFOSC &    2400 \\
2022-08-19.156 & 36.440 &       P60 &       SEDM &    1800 \\
2022-08-19.237 & 36.521 &     Shane &       Kast &    3360/3300 \\
2022-08-20.258 & 40.542 &      P200 &       DBSP &     600 \\
2022-08-22.201 & 42.485 &     Shane &       Kast &    3360/3300 \\
2022-08-28.182 & 48.466 &       P60 &       SEDM &    2250 \\
2022-08-29.157 & 49.441 &       P60 &       SEDM &    2250 \\
2022-09-01.142 & 52.425 &       P60 &       SEDM &    2250 \\
2022-09-04.211 & 55.494 &     Shane &       Kast &    3360/3300 \\
2022-09-08.852 & 60.136 &       NOT &     ALFOSC &    3600 \\
2022-09-23.241 & 74.525 &      Keck &       LRIS &    1200 \\
\enddata
\end{deluxetable}

==> tab_hostphot.tex <==
\begin{table}
\caption{Photometry of the host galaxy of SN\,2022oqm}\label{tab:host_phot}
\centering
%\scriptsize
\begin{tabular}{llc}
\toprule
Survey & Filter    & Brightness [AB mag] \\
\midrule
\galex	    &$	FUV	$&$	15.79	\pm	0.03	$\\
\galex	    &$	NUV	$&$	15.25	\pm	0.02	$\\
SDSS	    &$	u	$&$	14.09	\pm	0.04	$\\
SDSS	    &$	g	$&$	12.90	\pm	0.04	$\\
SDSS	    &$	r	$&$	12.29	\pm	0.03	$\\
SDSS	    &$	i	$&$	11.96	\pm	0.04	$\\
SDSS	    &$	z	$&$	11.73	\pm	0.03	$\\
Pan-STARRS	&$	g	$&$	12.90	\pm	0.03	$\\
Pan-STARRS	&$	r	$&$	12.29	\pm	0.02	$\\
Pan-STARRS	&$	i	$&$	12.05	\pm	0.01	$\\
Pan-STARRS	&$	z	$&$	11.90	\pm	0.03	$\\
Pan-STARRS	&$	y	$&$	11.69	\pm	0.08	$\\
\wise	    &$	W1	$&$	11.99	\pm	0.01	$\\
\wise	    &$	W2	$&$	12.52	\pm	0.02	$\\
\bottomrule
\end{tabular}
\tablecomments{All measurements are reported in the AB system and not corrected for reddening. %Non-detections are reported at $3\sigma$ confidence.
}
\end{table}
